Architecting Information Centric ETSI-M2M systems

The European Telecommunications Standards Institute (ETSI) released a set of specifications to define a restful architecture for enabling seamless service provisioning across heterogeneous Machine-to-Machine (M2M) systems. The current version of this architecture is strongly centralized, thus requiring new enhancements to its scalability, fault tolerance, and flexibility. To bridge this gap, herein it is presented an Overlay Service Capability Layer, based on Information Centric Networking design. Key features, example use cases and preliminary performance assessments are also discussed to highlight the potential of our approach.

==> autoICN.tex <==
Very futuristic vision of this new paradigm: possible services, main detail of the networkin operation, main implications,  pros and cons, [Alfredo+Madhi]

==> etsi.tex <==
ESTI M2M specifications define a generic and technology agnostic architecture for M2M services. Its main goal is to provide a framework for developing services independently of the underlying network, thus easing the deployment of vertical applications and making it possible an effective integration and interpretability of applications and data across industries. The standard includes service level requirements, architecture-level design, and protocol/API definition. It is articulated over two different tiers: device \& gateway domain, and network domain.% (see also Fig. \ref{etsi-m2m}).

The ETSI M2M architecture introduces the concept of Service Capabilities (SCs). SCs provide functions that are to be shared by different applications. SCs include application enablement, generic communication, reachability, addressing and repository, remote entity management, security, history and data Retention, transaction management, telco operator exposure, and interworking proxy. SCs can be deployed on an M2M network, a gateway, or a device.

An M2M Device runs M2M Applications using SCs. It is connected directly to the Network Domain via the Access network and may provide service to other devices connected to it that are hidden from the Network Domain. It can also be connected to the Network Domain via an M2M Gateway through the M2M Area Network. M2M Area Network provides connectivity between M2M Devices and M2M Gateways. M2M Gateway also runs M2M Applications using SCs, and acts as a proxy between M2M Devices and the Network Domain and may provide service to other devices connected to it that are hidden from the Network Domain \cite{Elmangoush:2012}.

Access network allows the M2M Devices and Gateways to communicate with the Core Network. M2M Service Capabilities Layer (SCL) provides M2M functions that can be shared by different Applications. It provides services through a set of open interfaces to manage subscriptions and notifications pertaining to events. M2M applications run the service logic and use SCs. Network Management Functions consist of all the functions required to manage the Access and Core Networks, such as Provisioning, Supervision, and Fault Management. M2M Management Functions consists of all the functions required to manage SCs in the Network Domain. 

Three reference points based on open APIs are specified: mIa, dIa, and mIa. The mIa reference point allows an application to access the M2M SCs in the M2M Core. dIa allows an application residing in a M2M Device to access the different M2M SCs in the same M2M Device or in a M2M Gateway; or an application residing in a M2M Gateway to access the different M2M SCs in the same M2M Gateway. The mId reference point allows an M2M Device or M2M Gateway to communicate with the M2M SCs in the M2M Core. These interfaces aim to be applicable to a wide range of network technology, so when specific potential bindings are defined, these bindings are not limiting the applicability when used in other networks using different protocols.

ETSI M2M adopted a RESTful architecture style, thus an SCL contains a resource tree where the information is kept. It standardized the resource structure that resides on an SCL as well as the procedure for handling the resources. A Resource is a uniquely addressable entity in the RESTful vocabulary. Each resource has a representation that shall be transferred and manipulated with the verbs. A resource shall be addressed using a Universal Resource Identifier (URI).  Operation on resource among Applications and SCLs, and between SCL instances are supported by means of Methods that constitute the communication on the mIa, dIa and mId interfaces. Each method conveys a set of information defined as Method Attributes.

An SCL resources tree includes different kind of resources such as sclBase, scls, scl, applications, application, etc. The SclBase resource contain all other resources of the hosting SCL. The scls resource is a collection that contains references of remote SCLs to which the hosting SCL is registered on.  the applications resource is a collection that contains references of applications which are locally registered on the hosting SCL. The application resource contains information about a registered local Application.

%\begin{figure}[htbp]
	%\centering
		%\includegraphics[width=8 cm]{etsi.eps}
	%\caption{ETSI M2M architecture.}
	%\label{etsi-m2m}	
%\end{figure}
%In Sec. \ref{distributed} a novel proposal in this direction will be formulated in order to: (1) fully exploit the benefits arising from the current centralized ETSI M2M design; (2) lower the load at the NSCL by enabling peer-to-peer interactions among the actors of an M2M ESTI system; (3) leverage caching capabilities already allowed by the standard using an ICN approach. 

%\textcolor{red}{Mahdi, please add security considerations.}


==> related.tex <==
The use of network overlays in M2M systems has been widely studied in literature with reference to many different facets. 

The proposals formulated in \cite{Kim:2010, Aucinas:2012, Bellavista:2013} mainly target performance optimizations in wireless mobile and sensor networks in order to speed up data transfer and lower energy consumptions. In \cite{Bellavista:2013}, it is proposed to exploit Mobile Ad hoc NETwork (MANET) overlays, autonomously and collaboratively formed over WSNs, to boost urban data harvesting in IoT. Such overlays are used to dynamically differentiate and speed up the delivery of urgent sensed data made available using the latest emergent standards/specifications for WSN data collection. In the context of mobile systems, in \cite{Aucinas:2012} it is proposed to map virtual clones of M2M nodes onto an overlay using a Cloud in order to let virtual clones to interact to each other thus minimizing the energy spent by wireless devices.
In \cite{Kim:2010} application level overlays are used to fasten the dissemination of urgent data in a WSN based on    
forest based topologies.


%A summary of the different problems faced so far along with corresponding approaches are reported in the sequel.
%
%%--- other papers (mobile networks, wsn)
%In \cite{Bellavista:2013}, it is proposed to exploit Mobile Ad hoc NETwork (MANET) overlays, autonomously and collaboratively formed over WSNs, to boost urban data harvesting in IoT. Such overlays are used to dynamically differentiate and speed up the delivery of urgent sensed data made available using the latest emergent standards/specifications for WSN data collection. In the context of mobile systems, in \cite{Aucinas:2012} it is proposed to map virtual clones of M2M nodes onto an overlay using a Cloud in order to let virtual clones to interact to each other thus minimizing the energy spent by wireless devices.
%In \cite{Kim:2010} application level overlays are used to fasten the dissemination of urgent data in a WSN based on    
%forest based topologies.

%--- DHT papers
On the other side, approaches conceived in \cite{Tanganelli:2013,Andreini:2010} are mainly devoted to resource discovery using structured overlays of proxy servers. In \cite{Tanganelli:2013}, it is proposed to build an overlay of proxy servers in a M2M deployment in order to handle resource discovery through P2P mechanisms. In particular, the location of a target resource is obtained by querying an overlay based on the eXtendible Metadata Hash Table (XMHT) \cite{Andreini:2010}, which is an extension of the widely used Pastry protocol \cite{pastry:2001}. This approach in itself is very valuable and deserves further investigations to understand to what extent it can fit complex M2M scenarios in which the level of popularity of different resources is highly heterogeneous. In fact,  from one hand, a Distributed Hash Table (DHT), which is the main element of this system, can be used to effectively locate rare items because its key-based routing is scalable. On the other hand, it may incur significantly higher overheads than unstructured approaches for popular content \cite{Lua:2005}. Also, at the present stage, a debate is still open about the effectiveness of DHT in very large scale systems \cite{jimenez2011,Crosby:2007}.

%--- HIP papers
Another branch of literature is mainly devoted at conceiving extensions to the well known Host Identity Protocol (HIP) \cite{HIP:2008}, which was originally proposed to handle Internet host identities and to decouple the host name space from the network address name space. In particular, a HIP-based M2M overlay network named HBMON is proposed in \cite{Dhraief:2012}. It extends the standard HIP in several directions in order to define, organize and manage device memberships within the overlay. Also HBMON proposes a novel IPv6 address assigning method in order to configure the overlay members with private IPv6 addresses. This architecture has been further improved in 
\cite{Dhraief:2013b} and \cite{Dhraief:2013} in order to embrace mobility and autonomic aspects too.

%XMPP 
The idea of using the eXtensible Messaging and Presence Protocol (XMPP) to discovery entities with a fully distributed approach in a M2M overlay has been discussed in \cite{Vaisanen:2012}. This service discovery protocol works at the application layer inside an XMPP client implementation. It can be categorized as an unicast protocol, as it sends direct discovery messages to known receivers. Its purpose is to discover M2M overlay entities presented as Jabber Identifiers (JIDs). In \cite{Latvakoski:2009} another interesting P2P approach to M2M residential home applications has been investigated too. These two latter approaches, albeit promising, has been conceived for dealing with simple M2M deployments and its effectiveness in large scale M2M systems deserves further analysis.

%.... DSON and SON ....
%The enhanced Dynamic Service Overlay Network (e-DSON) is proposed in \cite{Kim:2012} to handle service composition in context aware and user centric M2M applications. Basically the e-DSON could serve to orchestrate the usage of the data made available by a ETSI M2M system in order to allow the deployment of new services. 


%ICN papers
Last but not least, the idea of incorporating data awareness in M2M systems is being actively investigated and several ICN based proposals have been formulated \cite{Heidemann:2001, Okamoto:2012, Marias:2012, Rayes:2012, Trisha:13, Ravindran:2013, Batalla:2013}. The pioneering study in \cite{Heidemann:2001} demonstrated that attribute-named data at the lowest levels of communication can improve the energy efficiency of WSNs thanks to in-network processing with filters, data aggregation, and nested queries. Later on, when ICN architectures started being investigated worldwide, the idea to approach M2M systems using data centric networks lead to different interesting solutions and opened many implications \cite{Rayes:2012}. Noticeable contributions in \cite{Okamoto:2012} and \cite{Marias:2012} demonstrated the benefits arising from using an ICN approach in M2M systems, based on the the well known CCN \cite{Jacobson:09} and Publish Subscribe Internet Technology (PURSUIT) architectures \footnote{www.fp7-pursuit.eu/‎}, respectively. More specific applications of CCN in home networks has been presented in \cite{Ravindran:2013,Trisha:13,Batalla:2013}. 

Leveraging this important and thoughtful research path, the present contribution tries to move a further step forward in order to incorporate ICN capabilities in the emerging M2M ETSI standard. In this way, it will be possible to increase the scalability, the resilience, the flexibility, and the service availability of M2M deployments without loosing interoperability with respect to currently available M2M systems, which are compliant to the first release of the ETSI M2M standard. 

 





%\subsection{Information Centric Networking} [Alfredo]
%\textit{Host-centic} communication principles rule the Internet behavior and are at the basis of most standard applications (Web, Email, FTP, etc) mainly relying on well defined servers and hosts. However, the way users perceive network services has undergone through a substantial evolution during last years~\cite{Jacobson:09}. Nowadays, users ask for contents, regardless the physical location of the server, thus requiring novel networking primitives beyond the Internet Protocol (IP). In addition, the currect Internet suffers of a number of problems related to: (i) service provisioning across different wireless access technologies (i.e., mobility); (ii) security issues; (iii) environment with sporadic connectivity; (iv) network and server congestion, all deriving from the host -centric rationale.     
%
%The so called Information Centric Networking (ICN) promises to overtake these issues by posing contents at the core of networking primitives. In other words, according to the ICN paradigm, packet switching rules should be based on the contet to retrive rather than the host address from which the content could be downloaded.
%
%Several different ICN proposals have been formulated so far, whether based on hierarchical content names such as in NDN \cite{ndn:00} and CONVERGENCE \cite{Convergence:00} , or on flat self-certifying ones as in SAIL \cite{sail:00}, PURSUIT \cite{Fotiou:11} and DONA \cite{Koponen:07}, to name a few. 
%
%%At the time of this writing, the most compelling open issues in ICN research mainly refers to: caching strategies \cite{DBLP:conf/infocom/RossiR12,Fricker:2012:VAA:2414276.2414286}, routing schema \cite{Wang:12, Lee:11, Liu:12}, congestion control algorithms \cite{RAAQM:2013,CCTCP:2013}, and fast lookup engines \cite{Bari:12}, \cite{Varvello:12}.
%
%The idea of exploiting the ICN rationale in M2M systems is being investigated too  \cite{Heidemann:2001,Marias:2012,Trisha:13,Ravindran:2013} because M2M applications are inherently information centric, but all these proposals lack of a unifying and solid autonomic system that could ensure the Self-* properties that M2M systems should be based on. At the same time we remark that, to the best of authors' knowledge, while some early stage attempts are being formulated for envisaging autonomic services in ICN \cite{Pentikousis:2009,Sourlas:2012} no solid proposal does exist yet for handling the peculiar facets of M2M systems. Hence, the present contribution aims at discussing the open issues toward Autonomic Infomation Centric Networking (AICN) in M2M systems.

==> research.tex <==
[Alfredo+Mahdi]
